Designing Control Barrier Function via Probabilistic Enumeration for Safe Reinforcement Learning Navigation

Achieving safe autonomous navigation systems is critical for deploying robots in dynamic and uncertain real-world environments. In this paper, we propose a hierarchical control framework leveraging neural network verification techniques to design control barrier functions (CBFs) and policy correction mechanisms that ensure safe reinforcement learning navigation policies. Our approach relies on probabilistic enumeration to identify unsafe regions of operation, which are then used to construct a safe CBF-based control layer applicable to arbitrary policies. We validate our framework both in simulation and on a real robot, using a standard mobile robot benchmark and a highly dynamic aquatic environmental monitoring task. These experiments demonstrate the ability of the proposed solution to correct unsafe actions while preserving efficient navigation behavior. Our results show the promise of developing hierarchical verification-based systems to enable safe and robust navigation behaviors in complex scenarios.

==> sections/background.tex <==
\section{BACKGROUND AND PRELIMINARIES}
In this section, we cover the main foundations related to the research topics considered by our framework.

\subsection{Reinforcement Learning and Constrained Approaches}
Navigation tasks are typically modeled as a Markov decision process (MDP), represented by a tuple $<\mathcal{S},\mathcal{A}, R,\mathcal{P},\gamma>$ where $\mathcal{S} \in \mathbb{R}^d$ is the state space, $\mathcal{A}\in \mathbb{R}^2$ is the action space---which in this work consists of linear and angular velocities---$\mathcal{P}: \mathcal{S} \times \mathcal{A} \to \mathcal{S}$ is the
state transition function and $R: \mathcal{S} \times \mathcal{A} \to \mathbb{R}$ is a reward function. Given a stationary policy $\pi \in \prod$, an agent aims to maximize $J_{r}^{\pi} = \mathbb{E}_{\tau \sim \pi} \left[\sum_{t=0}^\infty \gamma^t R(s_t, a_t)\right]$, i.e., the expected discounted return for each trajectory $\tau = (s_0, a_0, \cdots, s_n,a_n)$, where $\gamma \in (0, 1]$ is a discount factor used to regulate the impact of future rewards. To consider safety, MDPs are typically extended to constrained MDPs (CMDPs) and incorporate a set of constraints during the training using one or more cost functions $C: \mathcal{S} \times \mathcal{A} \to [0, 1]$. Hence, constrained DRL algorithms aim at maximizing the expected return $J_r^{\pi}$ while maintaining costs under hard-coded thresholds $\mathbf{t}$:
$\max_{\pi \in \Pi} J_{r}^{\pi} \quad\text{s.t.}\quad J_{C}^{\pi} \leq \mathbf{t}$, with $J_{C}^{\pi} = \mathbb{E}_{\tau \sim \pi} [\sum_{t=0}^\infty \gamma^t C(s_t, a_t)]$. However, CMDPs present non-negligible limitations, such as the necessity of a parametrization of the policy (i.e., they are not applicable to value-based methods) \cite{Lagrangian}. To address such an issue, recent work  \cite{marchesini2023navigation} showed how incorporating penalties into the reward effectively influences policy toward safer behaviors while avoiding the limitations introduced by constrained approaches. Nonetheless, these methods only guarantee safety in expectation, making them unsuitable to ensure safe deployment.

\subsection{Formal Verification of Neural Networks}\label{prelim:FV}
%Neural network verification allows us to identify regions of the state space where desired safety properties hold. 

Given a trained policy represented by a neural network $\mathcal{N}: \mathcal{S} \to \mathcal{A}$, formal verification checks safety property defined in terms of input-output relationships for $\mathcal{N}$ \cite{LiuSurvey}. The general idea is to select a subset of the state space $\hat{\mathcal{S}} \subset \mathcal{S}$, define $\mathcal{Y}$ that specifies the desired (safe) output action for that portion of the state space and verify it. Fig. \ref{fig:safety_props} shows an explanatory example of a safety property for the aquatic navigation task. In detail, a FV tool propagates the intervals defined by $\hat{\mathcal{S}}$ through $\mathcal{N}$, performing a layer-by-layer reachability analysis to compute the output reachable set $\mathcal{R}(\hat{\mathcal{S}})$, i.e., the set of all possible outputs selected by the DNN for the region $\hat{\mathcal{S}}$. A tool then verifies whether $\mathcal{R}(\hat{\mathcal{S}}) \subseteq \mathcal{Y}$---indicating that the policy satisfies the safety property for all states in $\hat{\mathcal{S}}$. If even a single state $\bm{s}=[s_0,\ldots,s_n]^T \in \hat{\mathcal{S}}$ produces an output $a$ that falls outside $\mathcal{Y}$, the property is considered violated.  
However, due to the nonlinear nature of deep neural networks, determining whether such a violation exists is an NP-complete problem \cite{Reluplex}. Additionally, the binary nature of FV results (i.e., whether a violation occurs or not) does not provide sufficient safety information. For example, one model might exhibit only a small unsafe region around a specific counterexample, while another might have multiple widespread violations. To address the scalability and expressiveness of FV, recent works \cite{marzari2023dnn,marzari2024enumerating} propose to probabilistically enumerate all the portions of $\hat{\mathcal{S}}$ respecting or violating the safety desiderata, thus quantifying the rate at which agents either satisfy or not the DNN input-output relationships. We emphasize that, although the enumeration strategy used in our work is inherently probabilistic, its application to identifying unsafe regions reflects a conservative approach—misclassifying a portion of a safe area as unsafe is acceptable, whereas the opposite would compromise safety. In Sec. \ref{subsubsec: forward_inv} and \ref{subsubsec: cbf}, we will show how to exploit the enumeration results to design the CBF.

\subsection{Control Barrier Function}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/prop.png}
    \caption{Explanatory example of safety property for aquatic mapless navigation task. On the left, an unsafe state where the aquatic drone is near the left coastline to reach the target. On the right, the use of intervals, for each agent's input feature, allows the definition of a region of the state space $\hat{\mathcal{S}} \subset \mathcal{S}$ to verify that the agent in that region never selects an action corresponding to a left movement.}
    \label{fig:safety_props}
\end{figure}

Consider an affine nonlinear system of the form:  
\begin{equation}
\label{eq: affine_sys}
    \dot{x} = f(x) + g(x)u,
\end{equation}  
where $ x \in \mathcal{X} \subseteq \mathbb{R}^{n} $ represents the state variable within the dynamics model state space $\mathcal{X}$, and $ u \in \mathcal{U} \subseteq \mathbb{R}^{m} $ is the control input within the control input space $\mathcal{U}$. The functions $ f(x) $ and $ g(x) $ are nonlinear mappings from $ \mathbb{R}^{n} $ to $ \mathbb{R}^{n} $ and are assumed to be Lipschitz continuous. In this setting, a CBF is defined as follows.

\begin{definition}[Control Barrier Function \cite{cbf}]
\label{def: cbf}
    Let $\mathcal{C} \subset \mathbb{R}^{n}$ be the set defined by a continuously differentiable function $h: \mathbb{R}^{n} \rightarrow \mathbb{R}$ such that
    \begin{equation}
        \begin{split}
            \mathcal{C} &= \{x \in \mathbb{R}^{n}: h(x) \ge 0 \}, \\
            \partial\mathcal{C} &= \{x \in \mathbb{R}^{n}: h(x) = 0 \}, \\
            \text{Int}(\mathcal{C}) &= \{x \in \mathbb{R}^{n}: h(x) > 0 \}. \\
        \end{split}
    \end{equation}
We say that $h$ is a control barrier function if 
$\nabla h(x) \ne 0$ for all $x \in \partial\mathcal{C}$ and there exists a class-$\mathcal{K}$ function $\alpha$, such that for all $x \in \mathcal{C}, \exists u $ such that:
\begin{equation}
    L_{f}h(x) + L_{g}h(x)u \ge -\alpha(h(x)),
\end{equation}
with $L_{f}h(x):= \nabla h(x)^{T}f(x)$ and $L_{g}h(x):= \nabla h(x)^{T}g(x)$. 
\end{definition}

This formalization will be used in Sec \ref{subsubsec: cbf} to define the CBF for navigation policies.  
 
\subsection{Dynamic Models}
\label{subsec: dyn}

The design of the proposed pipeline requires the definition of the dynamic models in order to compute a corrective action for the navigation policy. Specifically, in this work, we consider (i) the kinematic equations of a mobile robot (Turtlebot3) and (ii) the nonlinear dynamics model of an aquatic drone. 
\subsubsection{Mobile robot}
\label{subsubsec: dyn_MB}
The kinematics equations of the robot are represented by:  
\begin{equation}
\dot{p}_x = v \cos{\theta}, \quad \dot{p}_y = v \sin{\theta}, \quad   \dot{\theta} = \omega,
\end{equation}
where $p_x, p_y, \theta$ are the positions and orientation of the robot and $v, \omega$ are the controlled linear and angular velocities.
 
\subsubsection{Aquatic drone}
\label{subsubsec: dyn_AD}
%The drone is described with the high nonlinear dynamic model. 
The aquatic drone motion is described following the 6-degrees-of-freedom nonlinear dynamic model, and the fluid dynamics coefficients are computed through spline interpolation using a high-fidelity simulator following common formalisms in the literature \cite{trotti2024towards, gierusz2016modelling}. Hence, the aquatic drone state and control vector are defined as:
\begin{equation} \label{eq:dyn_state}
    \begin{split}
    \bm{x} &= [v_1 \quad v_2 \quad v_3 \quad \omega_1 \quad \omega_2 \quad \omega_3 \quad p_{x} \quad p_{y} \quad p_{z} \quad \phi \quad  \theta \quad \psi]^{T},\\
    \bm{u} &= [\delta_{l} \quad \delta_{r}],
    \end{split}
\end{equation}
where $v_1, v_2, v_3$ are linear velocities and $\omega_1, \omega_2, \omega_3$ are the rate of the angles in the body frame, respectively. With $p_{x}, p_{y}, p_{z}$ and $\phi, \theta, \psi$, we refer to the boat position and the Euler angles in the Earth frame. Regarding the control variables, $\delta_l$ and $\delta_r$ represent the left and right thrusts of the boat.
The following equations express the linear accelerations along the three axes in the body frame:
\begin{equation}
\label{eq: lin_vel}
    \begin{split}
    \dot{v}_1 &= \frac{X}{m} - \omega_{2}v_3 + \omega_{3}v_2 - g  \sin(\theta), \\
    \dot{v}_2 &= \frac{Y}{m} - \omega_{3}v_1 + \omega_{1}v_3 + g  \sin(\phi)  \cos(\theta),\\
    \dot{v}_3 &=  \frac{Z}{m} - \omega_{1}v_2 + \omega_{2}v_1 + g  \cos(\phi)  \cos(\theta), 
    \end{split}
\end{equation}
with $X,Y,Z$ defined as:
\begin{equation}
\begin{tabular}{l c c}
$X = (\delta_r + \delta_l) - F_{x}$ & $\, \quad \,$ & $F_x =\frac{1}{2} \rho v_{1}^2 C_{Fx} A_x$,\\  
$Y = - F_{y}$ & $\, \quad \,$ & $F_y =\frac{1}{2} \rho v_{2}^2 C_{Fy} A_y$, \\
$Z = F_{b} - F_{z}$ & $\, \quad \,$ & $F_z = \frac{1}{2} \rho v_{3}^2 C_{Fz} A_z$.  \\
\end{tabular}
\end{equation}
In detail, $F_{b} = \rho g V_{\text{sub}}(p_z)C_b$ with $V_{\text{sub}}$ representing the submerged volume, $C_{Fx}, C_{Fy}, C_{Fz}, C_b$ are the drag coefficient on the translational tree axes and the bouncing drag respectively, while $A_x, A_y, A_z$ are the contact areas with the water.
The angular accelerations in the body frame are
\begin{equation}
    \begin{split}
        \dot{\omega}_{1} &= K + (c_1\omega_{2} +c_2\omega_{1})\omega_{2},\\
        \dot{\omega}_{2} &= M + (c_5\omega_{1})\omega_{3} - c_6(\omega_{1}^2 - \omega_{3}^2),\\
        \dot{\omega}_{3} &= N + (c_8\omega_{1}-c_2\omega_{3})\omega_{2},\\  
    \end{split}
\end{equation}
with $K,M,N$ expressed as: 
\begin{equation}
\label{eq: coeff_moment}
\begin{tabular}{l c c}
$K = - M_{x}- C_k(\phi)  F_{b}$ & $\, \quad \,$ & $M_x = \frac{1}{2} \rho \omega_{1}^2 C_{Mx} I_x$,\\  
$M = - M_{y} - C_m(\theta)  F_{b}$ & $\, \quad \,$ & $M_y = \frac{1}{2} \rho \omega_{2}^2 C_{My} I_y$, \\
$N = \frac{1}{2}(\delta_r - \delta_l)  d - M_{z}$ & $\, \quad \,$ & $M_z = \frac{1}{2} \rho \omega_{3}^2 C_{Mz} I_z$,\\
\end{tabular}
\end{equation}
where $C_{Mx}, C_{My}, C_{Mz}$ are the moment drag coefficient on the tree axes and $d$ is the distance between the two motors.
The time derivatives of the navigation equations in the Earth frame for each axis are given by
\begin{equation}
\label{eq: earthPose}
\begin{split}
    \dot{p}_{x} &= v_{1}\cos{\psi}\cos{\theta} + v_{2}(\cos{\psi}\sin{\theta}\sin{\phi} - \sin{\psi}\cos{\phi})\\
    & + v_{3}(\cos{\psi}\sin{\theta}\cos{\phi} + \sin{\psi}\sin{\phi}), \\
    \dot{p}_{y} &= v_{1}\sin{\psi}\cos{\theta} + v_{2}(\sin{\psi}\sin{\theta}\sin{\phi} + \cos{\psi}\cos{\phi})\\
    & + v_{3}(\sin{\psi}\sin{\theta}\cos{\phi} - \cos{\psi}\sin{\phi}), \\
    \dot{p}_{z} &= -v_{1}\sin{\theta} + v_{2}\cos{\theta}\sin{\phi} + v_{3}\cos{\theta}\cos{\phi}. \\  
\end{split} 
\end{equation}
Finally, the relationship between the angular velocities in the body frame and the Euler angular velocities in the Earth frame is defined by:
\begin{equation}
\label{eq: eulerAng}
    \begin{split}
        \dot{\phi} &= \omega_{1} + \tan{\theta}(\omega_{2}\sin{\phi} + \omega_{3}\cos{\phi}), \\
        \dot{\theta} &= \omega_{2}\cos{\phi} - \omega_{3}\sin{\phi}, \\
        \dot{\psi} &= \frac{\omega_{2}\sin{\phi} + \omega_{3}\cos{\phi}}{\cos{\theta}}.
    \end{split}
\end{equation}


==> sections/results_tab.tex <==
\begin{figure}[h!]

  % Second row
  \begin{minipage}[c]{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/tb3_results.png}
    %\fbox{\rule{0pt}{3cm} \rule{0.9\linewidth}{0pt}} % Placeholder box
  \end{minipage}%

  \vspace{1em}

  % Second row
  \begin{minipage}[c]{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/aquatic_results.png}
    %\fbox{\rule{0pt}{3cm} \rule{0.9\linewidth}{0pt}} % Placeholder box
  \end{minipage}%
 
  \caption{Training results using PPO, PPO\_penalty, and PPOLag on TB3 (top) and Aquatic (bottom) navigation task, respectively.}
  \label{fig: exp_results}
\end{figure}

==> sections/tabs.tex <==


\begin{table}[b]
     
  \caption{Evaluation results of the proposed verification-guided CBF on the trained policies over 100 trajectories.}
  \label{tab: tab_eval}
    \tiny
    \begin{tabular}{lcc|cc}
    
    &\multicolumn{2}{l}{\textbf{TB3 Evaluation}}&\multicolumn{2}{l}{\textbf{Aquatic Evaluation}}\\
    \toprule
    \textbf{Method} & \textbf{Success (\%)} & \textbf{Collision (\%)} & \textbf{Success (\%)} & \textbf{Collision (\%)}\\
    \hline
    PPO & 100$\pm$0 \% & 14.99 $\pm$0.02\% & 84.2 $\pm$ 9.75 \% & 11.22 $\pm$ 3.26 \%\\
    PPO+CBF & \textbf{100$\pm$0 \%} & \textbf{0$\pm$0\%} & \textbf{87.0 $\pm$ 12.72\%}& \textbf{0.0 $\pm$ 0.0} \% \\
     \hline
    PPO\_penalty & 100$\pm$0 \% & 3.32 $\pm$1.03\% & 89.7 $\pm$ 5.19 \% & 0.007 $\pm$ 0.005 \% \\
    PPO\_penalty+CBF & \textbf{100$\pm$0 \%} & \textbf{0$\pm$0\%} & \textbf{96.7 $\pm$ 2.30\%}& \textbf{0.0 $\pm$ 0.0} \%  \\
   \hline
    PPOLag & 99.66 $\pm$ 0.47\% & 0.47 $\pm$ 0.21\% & 84.0 $\pm$ 5.65 \% & 0.001 $\pm$ 0.002 \%\\
    PPOLag+CBF & \textbf{100$\pm$0 \%} & \textbf{0$\pm$0\%} & \textbf{94.0 $\pm$ 4.24\%}& \textbf{0.0 $\pm$ 0.0} \%\\
    \bottomrule
    \end{tabular}




 \end{table}
  



  % % Second row
  %   \vspace{0.5em}
  %    \tiny
  %   \begin{tabular}{lcc}
  %    \multicolumn{2}{l}{\textbf{Aquatic Evaluation}}&\\
  %   \toprule
  %   \textbf{Method} & \textbf{SR (\%)} & \textbf{CR (\%)} \\
  %   \midrule
  %   PPO & 84.2 $\pm$ 9.75 \% & 11.22 $\pm$ 3.26 \%\\
  %   PPO+CBF & \textbf{87.0 $\pm$ 12.72\%}& \textbf{0.0 $\pm$ 0.0} \%  \\
  %   \midrule
  %   PPO\_penalty & 89.7 $\pm$ 5.19 \% & 0.007 $\pm$ 0.005 \%\\
  %   PPO\_penalty+CBF & \textbf{96.7 $\pm$ 2.30\%}& \textbf{0.0 $\pm$ 0.0} \%  \\
  %   \midrule
  %   PPOLag & 84.0 $\pm$ 5.65 \% & 0.001 $\pm$ 0.002 \%\\
  %   PPOLag+CBF & \textbf{94.0 $\pm$ 4.24\%}& \textbf{0.0 $\pm$ 0.0} \% \\
  %   \bottomrule
  %   \end{tabular}
